Surprising lateral interactions between negatively charged adatoms on metal surfaces

Even something as conceptually simple as adsorption of electronegative adatoms on metal surfaces, where repulsive lateral interactions are expected for obvious reasons, can lead to unanticipated behavior. In this context, we explain the origin of surprising lateral interactions between electronegative adatoms observed on some metal surfaces by means of density functional theory calculations of four electronegative atoms (N, O, F, Cl) on 70 surfaces of 44 pristine metals. Four different scenarios for lateral interactions are identified, some of them being unexpected: (i) they are repulsive, which is the typical case and occurs on almost all transition metals. (ii,iii) They are atypical, being either attractive or negligible, which occurs on p-block metals and Mg, and (iv) surface reconstruction stabilizes the low-coverage configuration, preventing atypical lateral interactions. The last case occurs predominantly on s-block metals.

==> tables/Eb-table-hcp-lattices-001-fccSite.tex <==
\begin{threeparttable}
\begin{tabular}{l@{\hskip 0.4cm}cc@{\hskip 0.4cm}cc@{\hskip 0.4cm}cc@{\hskip 0.4cm}cc@{\hskip 0.4cm}}
  \hline
  ~\\[-0.98em]
Surface & \multicolumn{2}{@{\hskip -0.2cm}c}{$\mathrm{N_{ads}}$  } &  \multicolumn{2}{@{\hskip -0.2cm}c}{$\mathrm{O_{ads}}$ } &  \multicolumn{2}{@{\hskip -0.2cm}c}{$\mathrm{F_{ads}}$ } &  \multicolumn{2}{@{\hskip -0.2cm}c}{$\mathrm{Cl_{ads}}$ } \\
  & \tbt\ & \obo\  & \tbt\ & \obo\ & \tbt\ & \obo\ & \tbt\ & \obo\   \\
\hline
Be(001) & $ -4.79 $ & $ -3.16 $ & $ -6.59 $ & $ -5.51 $ & $ -4.49 $ & $ -4.51 $ & $ -2.89 $ & $ 0.63 $ \\  
Mg(001) & $ -6.22 $ & $ -6.74 $ & $ -6.98 $ & $ -7.48 $ & $ -5.84 $ & $ -6.08 $ & $ -4.12 $ & $ -3.89 $ \\  
Sc(001) & $ -7.93 $ & $ -7.28 $ & $ -9.16 $ & $ -9.07 $ & $ -6.98 $ & $ -6.73 $ & $ -5.37 $ & $ -5.10 $ \\  
Ti(001) & $ -8.07 $ & $ -7.50 $ & $ -8.90 $ & $ -8.31 $ & $ -6.54 $ & $ -6.46 $ & $ -5.10 $ & $ -4.44 $ \\  
Co(001) & $ -5.48 $ & $ -4.61 $ & $ -5.62 $ & $ -5.00 $ & $ -4.12 $ & $ -3.69 $ & $ -3.71 $ & $ -0.96 $ \\  
Zn(001) & $ -3.46 $ & $ -1.73 $ & $ -4.61 $ & $ -3.19 $ & $ -3.82 $ & $ -3.51 $ & $ -2.86 $ & $ -1.02 $ \\  
Y(001) & $ -7.69 $ & $ -7.06 $ & $ -9.03 $ & $ -8.99 $ & $ -6.94 $ & $ -6.69 $ & $ -5.38 $ & $ -5.27 $ \\  
Zr(001) & $ -8.05 $ & $ -7.76 $ & $ -8.84 $ & $ -8.41 $ & $ -6.46 $ & $ -6.41 $ & $ -5.09 $ & $ -4.90 $ \\  
Tc(001) & $ -6.05 $ & $ -5.19 $ & $ -6.02 $ & $ -5.76 $ & $ -4.27 $ & $ -3.94 $ & $ -4.02 $ & $ -2.16 $ \\  
Ru(001) & $ -5.45 $ & $ -4.65 $ & $ -5.38 $ & $ -4.98 $ & $ -4.03 $ & $ -3.54 $ & $ -3.85 $ & $ -1.81 $ \\  
Cd(001) & $ -2.69 $ & $ -1.18 $ & $ -4.05 $ & $ -2.94 $ & $ -3.86 $ & $ -3.63 $ & $ -2.92 $ & $ -1.80 $ \\  
Lu(001) & $ -8.03 $ & $ -7.32 $ & $ -9.44 $ & $ -9.35 $ & $ -7.08 $ & $ -6.78 $ & $ -5.35 $ & $ -5.25 $ \\  
Hf(001) & $ -8.43 $ & $ -8.13 $ & $ -9.22 $ & $ -8.77 $ & $ -6.54 $ & $ -6.49 $ & $ -5.08 $ & $ -4.90 $ \\  
Re(001) & $ -6.34 $ & $ -5.58 $ & $ -6.18 $ & $ -6.00 $ & $ -4.04 $ & $ -3.81 $ & $ -3.83 $ & $ -2.06 $ \\  
Os(001) & $ -5.40 $ & $ -4.77 $ & $ -5.27 $ & $ -4.92 $ & $ -3.66 $ & $ -3.98 $\tnote{a} & $ -3.52 $ & $ -1.70 $ \\  
Hg(001) & $ -1.29 $ & $ -1.75 $ & $ -3.03 $ & $ -3.06 $ & $ -3.18 $ & $ -2.93 $ & $ -2.24 $ & $ -2.05 $ \\  
Tl(001) & $ -3.44 $ & $ -2.66 $ & $ -4.14 $ & $ -3.87 $ & $ -4.14 $ & $ -4.13 $ & $ -3.19 $ & $ -2.94 $ \\  
\hline
\end{tabular}
\begin{tablenotes}
  \item{$^\mathrm{a}$} The adatom relaxed to the top site
\end{tablenotes}

\end{threeparttable}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../SupplementalMaterial"
%%% End:


==> tables/Eb-table-hcp-lattices-001-hcpSite.tex <==
\begin{threeparttable}
  
\begin{tabular}{l@{\hskip 0.4cm}cc@{\hskip 0.4cm}cc@{\hskip 0.4cm}cc@{\hskip 0.4cm}cc@{\hskip 0.4cm}}
  \hline
  ~\\[-0.98em]
Surface & \multicolumn{2}{@{\hskip -0.2cm}c}{$\mathrm{N_{ads}}$  } &  \multicolumn{2}{@{\hskip -0.2cm}c}{$\mathrm{O_{ads}}$ } &  \multicolumn{2}{@{\hskip -0.2cm}c}{$\mathrm{F_{ads}}$ } &  \multicolumn{2}{@{\hskip -0.2cm}c}{$\mathrm{Cl_{ads}}$ } \\
  & \tbt\ & \obo\  & \tbt\ & \obo\ & \tbt\ & \obo\ & \tbt\ & \obo\   \\
\hline
Be(001) & $ -5.12 $ & $ -3.25 $ & $ -6.84 $ & $ -5.53 $ & $ -4.63 $ & $ -4.38 $ & $ -2.94 $ & $ 0.63 $ \\  
Mg(001) & $ -5.81 $ & $ -5.60 $ & $ -7.42 $ & $ -7.60 $ & $ -5.84 $ & $ -6.04 $ & $ -4.12 $ & $ -3.85 $ \\  
Sc(001) & $ -8.37 $ & $ -8.37 $ & $ -9.30 $ & $ -9.29 $ & $ -6.87 $ & $ -6.66 $ & $ -5.33 $ & $ -5.07 $ \\  
Ti(001) & $ -8.01 $ & $ -7.58 $ & $ -8.62 $ & $ -8.19 $ & $ -6.33 $ & $ -6.28 $ & $ -5.02 $ & $ -4.35 $ \\  
Co(001) & $ -5.68 $ & $ -4.66 $ & $ -5.68 $ & $ -5.01 $ & $ -4.19 $ & $ -3.75 $ & $ -3.71 $ & $ -0.96 $ \\  
Zn(001) & $ -3.53 $ & $ -1.76 $ & $ -4.73 $ & $ -3.19 $ & $ -3.85 $ & $ -3.49 $ & $ -2.89 $ & $ -1.01 $ \\  
Y(001) & $ -8.12 $ & $ -8.25 $ & $ -9.10 $ & $ -9.17 $ & $ -6.82 $ & $ -6.60 $ & $ -5.35 $ & $ -5.24 $ \\  
Zr(001) & $ -7.95 $ & $ -7.82 $ & $ -8.53 $ & $ -8.21 $ & $ -6.32 $ & $ -6.25 $ & $ -5.11 $ & $ -4.84 $ \\  
Tc(001) & $ -6.46 $ & $ -5.40 $ & $ -6.56 $ & $ -6.09 $ & $ -4.49 $ & $ -4.08 $ & $ -4.03 $ & $ -2.26 $ \\  
Ru(001) & $ -6.19 $ & $ -4.87 $ & $ -5.98 $ & $ -5.13 $ & $ -3.93 $ & $ -3.59 $ & $ -3.80 $ & $ -1.72 $ \\  
Cd(001) & $ -2.75 $ & $ -1.19 $ & $ -4.13 $ & $ -2.93 $ & $ -3.87 $ & $ -3.62 $ & $ -2.96 $ & $ -1.78 $ \\  
Lu(001) & $ -8.52 $ & $ -8.59 $ & $ -9.58 $ & $ -9.55 $ & $ -6.95 $ & $ -6.70 $ & $ -5.29 $ & $ -5.21 $ \\  
Hf(001) & $ -8.34 $ & $ -8.28 $ & $ -8.77 $ & $ -8.49 $ & $ -6.20 $ & $ -6.21 $ & $ -4.93 $ & $ -4.78 $ \\  
Re(001) & $ -6.79 $ & $ -5.81 $ & $ -6.77 $ & $ -6.47 $ & $ -4.27 $ & $ -3.90 $ & $ -3.85 $ & $ -2.15 $ \\  
Os(001) & $ -6.15 $ & $ -5.08 $ & $ -5.79 $ & $ -5.04 $ & $ -3.50 $ & $ -3.98 $\tnote{a} & $ -3.42 $ & $ -1.60 $ \\  
Hg(001) & $ -1.98 $ & $ -1.87 $ & $ -3.03 $ & $ -3.10 $ & $ -2.46 $ & $ -2.78 $ & $ -1.75 $ & $ -2.01 $ \\  
Tl(001) & $ -3.29 $ & $ -2.70 $ & $ -4.24 $ & $ -3.87 $ & $ -4.10 $ & $ -4.14 $ & $ -3.15 $ & $ -2.93 $ \\  
\hline
\end{tabular}
\begin{tablenotes}
\item{$^\mathrm{a}$} Adatom relaxed to the (more stable) top site
\end{tablenotes}
\end{threeparttable}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../SupplementalMaterial"
%%% End:


==> tables/atest.tex <==
\begin{tabular}{l@{\hskip 0.4cm}cc@{\hskip 0.4cm}cc@{\hskip 0.4cm}cc@{\hskip 0.4cm}cc@{\hskip 0.4cm}}
  \hline
  ~\\[-0.98em]
Surface & \multicolumn{2}{@{\hskip -0.2cm}c}{\Eb($\mathrm{N_{ads}}$)  } &  \multicolumn{2}{@{\hskip -0.2cm}c}{\Eb($\mathrm{O_{ads}}$)  } &  \multicolumn{2}{@{\hskip -0.2cm}c}{\Eb($\mathrm{F_{ads}})$ } &  \multicolumn{2}{@{\hskip -0.2cm}c}{\Eb($\mathrm{Cl_{ads}}$) } \\
  & \tbt\ & \obo\  & \tbt\ & \obo\ & \tbt\ & \obo\ & \tbt\ & \obo\   \\
\hline
Al(100) & $-6.419$ & $-5.941$ & $-7.293$ & $-7.711$ & $-4.780$ & $-4.945$ & $-3.332$ & $-2.399$ \\
Ca(100) & $-7.194$ & $-7.243$ & $-8.355$ & $-7.934$ & $-6.861$ & $-6.802$ & $-5.285$ & $-5.274$ \\
Ni(100) & $-5.333$ & $-3.779$ & $-5.358$ & $-3.872$ & $-3.903$ & $-3.167$ & $-3.574$ & $-0.633$ \\
Cu(100) & $-3.930$ & $-2.204$ & $-4.669$ & $-2.799$ & $-3.864$ & $-3.021$ & $-3.356$ & $-0.914$ \\
Sr(100) & $-6.532$ & $-6.424$ & $-8.059$ & $-7.464$ & $-6.824$ & $-6.711$ & $-5.345$ & $-5.314$ \\
Rh(100) & $-5.352$ & $-4.131$ & $-5.048$ & $-4.248$ & $-3.580$ & $-2.910$ & $-3.492$ & $-1.371$ \\
Pd(100) & $-4.693$ & $-3.291$ & $-4.279$ & $-3.178$ & $-3.158$ & $-2.463$ & $-3.162$ & $-1.418$ \\
Ag(100) & $-2.343$ & $-1.158$ & $-3.467$ & $-1.932$ & $-3.589$ & $-2.766$ & $-3.092$ & $-1.705$ \\
In(100) & $-3.608$ & $-3.849$ & $-4.859$ & $-5.126$ & $-4.183$ & $-4.210$ & $-3.088$ & $-2.832$ \\
Sn(100) & $-4.053$ & $-4.220$ & $-4.942$ & $-5.002$ & $-3.895$ & $-3.897$ & $-2.936$ & $-2.641$ \\
Ir(100) & $-5.164$ & $-4.217$ & $-4.758$ & $-3.980$ & $-3.117$ & $-3.247$ & $-3.040$ & $-1.996$ \\
Pt(100) & $-4.833$ & $-3.645$ & $-4.177$ & $-3.127$ & $-2.612$ & $-2.603$ & $-2.701$ & $-1.145$ \\
Au(100) & $-2.679$ & $-1.483$ & $-3.051$ & $-1.707$ & $-2.706$ & $-2.154$ & $-2.395$ & $-1.294$ \\
Pb(100) & $-3.389$ & $-3.080$ & $-4.479$ & $-4.633$ & $-4.025$ & $-3.996$ & $-3.074$ & $-2.813$ \\
\hline
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../SupplementalMaterial"
%%% End:

